embComp: Visual Interactive Comparison of Vector Embeddings

This paper introduces embComp, a novel approach for comparing two embeddings that capture the similarity between objects, such as word and document embeddings. We survey scenarios where comparing these embedding spaces is useful. From those scenarios, we derive common tasks, introduce visual analysis methods that support these tasks, and combine them into a comprehensive system. One of embComp's central features are overview visualizations that are based on metrics for measuring differences in the local structure around objects. Summarizing these local metrics over the embeddings provides global overviews of similarities and differences. Detail views allow comparison of the local structure around selected objects and relating this local information to the global views. Integrating and connecting all of these components, embComp supports a range of analysis workflows that help understand similarities and differences between embedding spaces. We assess our approach by applying it in several use cases, including understanding corpora differences via word vector embeddings, and understanding algorithmic differences in generating embeddings.

==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by $Author: jpeltier $ $Date: 2007-04-03 16:51:34 -0700 (Tue, 03 Apr 2007) $
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers
according to the specifications for submission to conferences sponsored
by the IEEE Visualization & Graphics Technical Committee (VGTC). This
includes:

Conferences that use the 'conf' document option:
- IEEE Virtual Reality
- IEEE Symposium on 3D User Interfaces
- Symposium on Haptic Interfaces for Virtual Environment and Teleoperator Systems
- IEEE Symposium on Asia Pacific Visualisation
- IEEE Symposium on Interactive Ray Tracing
- IEEE Symposium on Visual Analytics Science and Technology
- IEEE Symposium on Visual Analytics Science and Technology
- IEEE Visualization Conference (Posters Only)
- IEEE Information Visualization Conference (Posters Only)
- IEEE Symposium on Volume Graphics

It contains 11 files/directories:

README          - this file
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default conference mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> README_IEEEtran <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> tex/conclusion.tex <==
This is the conclusion of the paper.

==> tex/designs.tex <==
\label{sec:design}
To help users address the tasks discussed in \S\ref{sec:example_scenarios}, we have created a flexible, interactive system that allows a user to select views and combine them in informative ways. 

Many tasks involve working with subsets of objects in the embedding.
Users need to identify interesting subsets of objects, explore them in detail, and connect them back to the overall embedding and to downstream outcomes (e.g., clustering results).
To support this need, our system has a notion of a \emph{selection set}.
The selection set may be created using a summary view (e.g., clicking in the green box at the middle right of Figure~\ref{fig:overlap_ex1}), and is displayed across all active summary views (e.g., Figures~\ref{fig:overlap_ex1}, \ref{fig:spread_ex1}, \ref{fig:pdist_ex3}).
Other \emph{mezzo-scale} views are specifically designed to support detailed examination and interaction with the set.

Our system supports a number of mechanisms to help the user build selection sets.
Interacting with regions of summary displays provides an efficient way to specify objects with a particular property, such as objects with low overlap. 
The system allows for set arithmetic to combine these specifications, for example to union sets together or to intersect sets to create conjunctive queries (e.g., items with low overlap and high density, or items with low spread in one embedding and high spread in the other).
The system maintains a history of prior selection sets, allowing a user to return to previous work, or use them in combination.

The selection list view provides fine grained specification and viewing of the selection set.
Data and meta-data about the selected objects are shown in a sortable, searchable, and filterable table, which may be used to select a subset of the current selection.
This allows for the creation of selection sets of the user's interests (e.g., objects they are researching) by selecting a large set (or all items) and searching and filtering appropriately.

The metrics have different forms and serve different tasks, and therefore, each require specialized views.
Additionally, the views must all be designed to support selection set interactions in addition to conveying the metrics.
Therefore, the views have been carefully selected, although their visual designs are not novel.  

\subsection{Overviews of Rank Metrics}
\label{sec:design-rank}
The overlap and spread metrics (\S\ref{sec:measures}) provide an integer value for each object.
Overviews of the distribution of these metrics over the set of objects show the set of objects with each value (Figures~\ref{fig:overlap_ex1}, \ref{fig:spread_ex1}, \ref{fig:pdist_ex3}).
To provide for a scalable overview, we show only the count for each value.
While a bar chart would be the conventional choice for such data (and is provided as an option), we prefer a color map display as it scales better to high densities (e.g., Figure~\ref{fig:overlap_ex1}) and provides screen area even for low values.
This is important because low values are often interesting for both display but also selection.
Both boxplots and color encodings associate screen areas with sets of objects, making them function for both selection display (the rectangle is highlighted whenever its contents intersect the selection set) and specification (clicking on the rectangle selects the items). 

For both overlap and spread, views show the distributions for a user selectable range of neighborhood sizes.
The distributions are shown juxtaposed (e.g., Figures~\ref{fig:overlap_ex1}, \ref{fig:spread_ex1}, \ref{fig:pdist_ex3}). 

The overlap and spread metrics require subtly different visual designs.
Overlap has one value per object, whereas spread has a different value for each embedding.
In the \emph{spread view} (Figure~\ref{fig:spread_ex1}), the distribution for both embeddings may be shown together for each neighborhood size, facilitating comparison between distributions, or the distributions may be grouped to show the different sizes for each embedding to facilitate assessment of the individual embeddings.
Overlap distributions have the property that the number of possible values depends on the size of the neighborhood.
The \emph{overlap view} provides an axis-filling design (Figure~\ref{fig:overlap_ex1}), although fixed sizes for the bins is also available.

\subsection{Overviews of Distance Metrics}
\label{sec:design-distance}
While distances cannot be compared directly between embeddings (see \S\ref{sec:example_scenarios}), overviews of distance metrics for each embedding are used to make aggregate comparisons and to compare selection sets with other objects in each embedding (e.g., Figure~\ref{fig:pdist_ex3}).
The designs for overviews of distance metrics are similar to those for rank metrics, however, they must handle the continuous distance values (as opposed to discrete ranks) by binning.
The \emph{neighborhood distance view} (Figure~\ref{fig:ndistance_ex2}) is similar to the spread view, with the y-axis representing bins of different distances, and the counts representing the number of objects with their $n^{\text{th}}$ nearest neighbor having that distance apart.
The \emph{density view} %(Figure~\ref{fig:density}) 
is visually similar, except that distributions (along the x-axis) are chosen for different radius distances.
The y-axis represents counts within the ball of that radius (the density), and the encoded value is the number of objects that have the density (y-value) for the particular ball size (x-value).

The pairwise metrics, distances and stress, differ from other metrics in that they provide a value for each edge (pair of objects), rather than for each object.
To overview these metrics, the \emph{pairwise distance view} (Figure~\ref{fig:pdist_ex3}) and \emph{stress view} provide histograms showing the distribution of edge lengths.
A separate histogram is overlayed for the selection set, allowing the distribution of values within the set to be compared with the overall distribution.
Unlike other overviews, these histograms do not allow for set specification.

\subsection{Detail Views of Selections and Objects}
\label{sec:design-detail}
Two views provide details on the selection set.
The selection list, described above, provides a tabular view for reading details and filtering.
A \emph{neighborhood wall} view (Figure~\ref{fig:wall_ex2}) shows the change for each neighbor of each object in the selection.
The view presents a grid of squares, with each column representing the neighbors of a member of the selection ordered by rank.
Each square is colored according to its rank in the other embedding. 

Other views provide detailed information for the focus object.
A \emph{textual description} view details available information about the focus object.
A \emph{neighbor list} view provides a tabular representation of the neighbors of the object in each embedding.
The \emph{buddy plot} view uses the buddy plot design~\cite{Alexander2016} to show the neighbors of the focus object in a compact visual form.
The neighbors of an object are shown as in a row for each embedding and colored by their rank in the other embedding.
The buddy plot can be configured to show rank or distance information, as described in~\cite{Alexander2016}. 

\subsection{Context Views}
\label{sec:design-context}
Our system provides views that provide context for the differences between embeddings.
They show how these differences lead to different results in the outputs of usages of the embeddings.
The \emph{clustering} view runs a clustering algorithm (either k-Means or DBSCAN~\cite{Ester1996}) on each embedding and compares the results as a confusion matrix.
The system matches similar clusters between embeddings to order the matrix to best show the degree of similarity.
The confusion matrix also allows for inspection of the differences: squares of the confusion matrix can be selected to inspect how they differ in other views of the embedding comparison.

%\begin{figure}
%	\centering
%	\includegraphics[width=.6\columnwidth]{pictures/cluster_glove_sg_eebo.png}
%	\caption{ An example of the cluster comparison matrix.
%					   }
%	\label{fig:cluster_matrix}
%\end{figure}

The \emph{scatterplot view} displays a 2D visualization of the embedding spaces (Figure~\ref{fig:scatter_ex1}).
If the embeddings are 2D, they are shown directly, otherwise dimensionality reduction is used to embed the embeddings into 2D.
The system supports t-SNE, LLE, IsoMap, MDA, and PCA for dimensionality reduction.
The scatterplot view allows for display and specification of the selection set, providing the user with the ability to see a context of what is close to the selection set in each embedding. When the scatterplot view is used with topic models, it offers the option of creating \emph{psuedo-documents} for each topic, placed in the embedding with 100\% content of the topic. These documents provide locations in the dimensionality reduced embeddings that show where a topic is focused (see Figure~\ref{fig:topics-scatter} for an example).


==> tex/measures.tex <==
At the core of our approach is a set of metrics that quantify similarities and differences between embeddings based on a range of object-local and global \todo{TM: should be 'based on a range of local and global object properties'} properties.
This allows us to create aggregate, visual overviews of these properties that provide effective summaries of how well two embeddings correspond.
In this section, we list all metrics we have found to be useful while designing and using our approach \todo{change to 'useful in our case studies'} , and connect them back to the tasks and scenarios discussed previously (\S\ref{sec:tasks_and_requirements}). \todo{don't use the paragraph symbol, just use 'section N'}
For this, we first start with a few basic definitions, and then go on to define our metrics.

Since we are not using the actual dimensions of the embedding space as part of our metrics, \todo{this makes no sense: if you do NOT need the actual dimensions for your metric, you really don't need an embedding at all.} we can define an embedding $e$ as a set of items with a corresponding function $d_e$ that defines a positive distance between each pair of objects in the embedding
\[
\forall i, j \in e: d_e(i, j) \ge 0
\]
Object $i$ is a \emph{neighbor} of object $j$ in embedding $e$ if and only if $i\in e\land j\in e\land i\ne j$.
We define the $n$-neighborhood of object $i$ in embedding $e$ as
\[
	neighborhood_e(n, i) = \argmin_{\substack{|S| = n\\S\subseteq e\backslash i}}{\sum_{j\in S}{d_e(i,j)}}
\]

\todo{sorry, but this definition is incorrect. To properly (mathematically) define it, one needs to first create a ranking of items and then create a set that is cut off at item n. However, I think this mathematical definition is overkill, unless you specifically need it somewhere again?!}

In other words, for an object $j$, $j\in neighborhood_e(n,i)$ if $j$ is among the $n$ objects with the lowest distance to $i$ in $e$. \todo{this verbal definition is all that is needed, imho}
\todo{This is actually not how we treat neighborhoods in the implementation, but I can't come up with a good way of defining what we do in the system.}
An item $j$ has rank $n$ in the neighborhood of $i$ in $e$ if and only if $j$ is in the $n$-neighborhood of $i$ in $e$, but not in the $(n-1)$-neighborhood of $i$ in $e$.
We define the function $rank_e(i,j)$ to represent the rank of object $j$ in the neighborhood of object $i$ in embedding $e$, and $q_e(n, i)$ the neighbor $j$ of $i$ in $e$ that satisfies $rank_e(i,j) = n$.
In other words, $q_e(n, i)$ is the $n^{th}$ nearest neighbor of $i$ in embedding $e$.
\todo{We have to define multiple ones here. How do we resolve this?}
Based on these definitions, we can now define our metrics.

\noindent\textbf{Overlap} is a symmetric metric that measures the size of the overlap between object neighborhoods of a certain size in both embeddings.
We define overlap as
\[
	overlap_{e_1,e_2}(n, i) = | neighborhood_{e_1}(n, i) \cap neighborhood_{e_2}(n, i) |
\]
The distribution of overlaps between object representations in two embeddings give us insight into how consistently objects keep their neighbors across embeddings.
This metric is one of our core ones and it plays a significant role for most of the tasks, in particular \textbf{tasks 1, 2, 3, and 7}.
Viewing a succession of overlap distributions for different neighborhood sizes $n$ can provide insights into how well embeddings correspond.
For example, we might learn from it, that a tSNE reduction of a topic model is able to by and large keep documents close to their five nearest neighbors in the original space.

\noindent\textbf{Spread} measures to what extent neighborhoods stay compact across embeddings.
It is a non-symmetric metric that offers additional insight into what happens to neighborhoods from one of the embeddings in the second embedding.
We use three version of spread.
The first one is called \emph{singular spread} and is defined as
\[
	spread\_s_{e_1,e_2}(n, i) = rank_{e_2}(i, q_{e_1}(n, i))
\]
The second version is called \emph{neighborhood-max} and is defined as
\[
	s\_max_{e_1,e_2}(n, i) = max( rank_{e_2}(i, q_{e_1}(1, i)), \ldots, rank_{e_2}(i, q_{e_1}(n, i)) )
\]
A third version, \emph{neighborhood-median} uses the median instead of the max within a neighborhood
\[
	s\_med_{e_1,e_2}(n, i) =\\median( rank_{e_2}(i, q_{e_1}(1, i)), \ldots, rank_{e_2}(i, q_{e_1}(n, i)) )
\]
Singular spread provides insight into how a rank changes from one embedding to the next. This measure is not symmetric.
%neighbors of a specific rank move across the embeddings.
%As spread is not symmetric, we have two distributions per $n$ and embeddings pair.
It supports tasks with a focus on analyzing differences in the neighborhood representations, such as \textbf{tasks 1, 3, 5, and 6}.
The neighborhood-max and neighborhood-median versions focus on the characterization of the maximum and average changes in the neighborhood respectively. Both versions support different types of tasks. While neighborhood-max is well suited for \textbf{tasks 2, 4, 5, and 9}, neighborhood-median might be better suited for \textbf{2, 3, 4, and 6}, which involve comparing embedding versions for the same dataset. \todo{ok, I take it for face value, but it is not necessarily clear here}
%The neighborhood-max version provides insight into how extreme the changes that happen between neighborhoods are.
%If there are neighbors that move really far, it might indicate some significant changes in a neighborhood.
%It helps is relevant for tasks where large changes in neighborhoods might be relevant, such as \textbf{tasks 2, 4, 5, and 9}.
%The neighborhood-median version conveys a sense of the average movement in the neighborhoods instead of focusing on the worst cases.
%It is particularly useful for tasks such as \textbf{2, 3, 4, and 6} that involve comparing embedding versions for the same dataset.

Torsten: I'd prefer a 'todo' function that doesn't move things into the margin. I don't know how to do this. If there is an easy way, please let me know. The following doesn't make sense in the margins:

I suggest to change your notation, such that it is easier to read.
\begin{itemize}
\item I am fine with $\text{neighborhood}_e(n,i)$ as long as you do not italize it. I still would rather prefer $\text{neighborhood}_{e,n}(i)$.
\item I suggest to introduce the following notation: $s_0(i), s_1(i), s_2(i), ..., s_n(i)$ as a list of all elements sorted by their distance to $i$. I.e. $s_0(i)=i$ If it is not clear from the context, use $s_0^e(i), s_1^e(i), s_2^e(i), ..., s_n^e(i)$
\item Now you can easily explain $\text{neighborhood}_{e,n}(i)$.
\item change $rank_e(i,j)$ to $rank_{e}^i(j) = n$ is and only if $j=s_n(i)$ given embedding $e$.
\item please don't use $q_e(n,i)$ it is really hard to parse. Instead use $s_n^e(i)$.
\item now your spread simply becomes $rank_{e_2}^i(s_n^{e_1}(i))$
\end{itemize}


% order\\

\noindent\textbf{Average n-ball density} is a metric that provides insight into one embedding at a time.
Comparisons between embeddings are made by comparing visualizations of these distributions.
The metric is defined as the number of neighbors of an object within the distance of the average $n$-neighbors of the entire embedding
\[
	n\_density_e(n, i) = | \{ j | d_e(i, j)\leq mean_e(n) \} |
\]
with
\[
	mean_e(n) = \frac{\sum_{i\in e}d_e(i, q_e(n,i))}{|e|}
\]
Average n-ball density provides insight into how dense the local source around an object is.
By expressing this density as neighbor counts within embedding-specific radii that adapt to the average distances of each embedding, the resulting notion of density remains comparable across embeddings.
This metric helps in particular for higher dimensional data where distances tend to be less meaningful than densities, such as \textbf{tasks 9, 4, and 2}.

\noindent\textbf{Neighbor Distance} is the distance of an object to its $n$-neighbor:
\[
	n\_dist_e(n, i) = dist_e(i, q_e(n, i))
\]
\todo{What is $dist_e$? do you mean $d_e$?}
Like the previous metric, this is also embedding-specific, and comparisons are made by comparing distributions and single values across embeddings.
The distances of an item to its nearest neighbor, in relation to the distribution of distances within the entire embedding helps gauge the significance of the neighborhood relationship.
This is particularly helpful in gauging how meaningful neighborhood relations are in lower dimensional embeddings, in which distances tend to be more tangible than densities, such as \textbf{tasks 1, 3, and 8}.

\noindent\textbf{Pairwise Distance} for an embedding $e$ is the distance $d_e$ defined for each pair $i,j\in e$ of instances.
Again, this metric is embedding-specific.
It is useful for interpreting object sets, particularly in higher-dimensional embeddings, relative to the entire embeddings (e.g., for \textbf{tasks 4, 7, and 9}).
For example, it can be helpful in gauging how central a set of objects is within the embedding.
In addition, comparing shape of the distribution provides insight into how the objects are spread out within two embeddings and whether there are differences between them in terms of object distribution within the space.
Comparisons can be made between the distribution of these distances across embeddings, which provides insight into the distribution of objects across the embedding.
In addition, comparing the distribution of a subset of objects to all others in an embedding can help understand of how central the selected group of objects is on average within the embedding.

\noindent\textbf{Strain} measures the difference in distance between each pair of object in the two embeddings.
We define strain as
\[
	strain_{e_1,e_2}(i,j) = \log{\frac{d_{e1}(i,j)}{d_{e2}(i,j)}}
\]
It is a metric that is used a lot and in various versions to measure the accuracy of dimensionality reductions compared to their source embedding (e.g., \textbf{tasks 6 and 7}).
Sometimes this metric is also called \emph{stress}.
In fact, there is a whole family of dimensionality reduction methods that aim to minimize strain to create dimensionality reductions (see \S\ref{sec:related_work_embeddings}).
The version we use is based on the fraction of distances between a pair of objects in two embeddings.
Taking the $log$ has two effects: (1) It dampens the effect of relative large differences and reduces the range of the resulting scale used to represent them, and (2) it introduces a symmetry between differences in both embeddings with negative values for $d_{e1}(i,j)<d_{e2}(i,j)$ and positive values for $d_{e1}(i,j)>d_{e2}(i,j)$.
While strain is a good metric to gauge the overall fit between to embeddings, it overemphasizes distances between objects that are far away from each other in both embeddings, and for whom the absolute distances, depending on the type of embeddings, might not be that relevant.
Still, in combination with the other metrics it provides useful insight, in particular when comparing the distribution of strain of a subset of instances to the entire distribution,a nd we found it to be useful for most of the tasks. \todo{last sentence is not a sentence.}



==> tex/measures_v2.tex <==
At the core of our approach is a set of metrics that quantify similarities and differences between embeddings based on a range of local and global properties.
%This allows us to create aggregate, visual overviews of these properties that provide effective summaries of how well two embeddings correspond.
In this section, we list %all
metrics we have found useful, % in our case studies,
and connect them back to the scenarios from \S\ref{sec:tasks_and_requirements}.

To provide notation, we define $E$ as the set of objects in an embedding $e$, and $d_{e}(i,j) \geq 0$ as the distance between two objects $i\in E$ and $j\in E$.
Every embedding can have a different distance metric defined for its objects.
In practice, we use either Euclidean or cosine distance in our use cases.
The list $s_0^e(i), s_1^e(i), s_2^e(i), ..., s_n^e(i)$ contains all elements sorted by their distance to $i$ in $e$.
The n-neighborhood of an object $i$ in embedding $e$ is defined as follows: $j\in \mathrm{neighborhood}_{e,n}(i) = s_0^e(i), ..., s_n^e(i)$.
An item $j$ has rank n, $rank_e^i(j) = n$, if and only if $j=s_n^e(i)$ in embedding $e$.
Based on these definitions, we can now define our metrics.

\subsection{Per-Object Comparison of Structure}
	\label{sec:measures-rank}
This category of metrics assesses the amount of change in the neighborhood of a specific object considering only rank.
When coupled with summary views (\S\ref{sec:design-rank}), these metrics are a starting point for assessing the amount of change between embeddings and identifying sets of objects with interesting changes or similarities.

\noindent\textbf{Overlap} measures the number of common neighbors of an object in both embeddings for neighborhoods of a certain size.
The distribution of overlaps between object embeddings provides insight into how consistently objects keep their neighbors across embeddings.
This metric plays a significant role for most of the scenarios, e.g.,~\exhdtored, \exhypp, \exvecsz and \exoverfit, and we often use it as an entry point in our case studies.
Viewing a succession of overlap distributions for different neighborhood sizes $n$ can provide insight into how well embeddings correspond.
For example, we might learn from it, that a t-SNE reduction of a topic model is able to by and large keep documents close to their five nearest neighbors in the original space (\exhdtored).
We define overlap as
\[
	overlap_{e_1,e_2}(n, i) = | \mathrm{neighborhood}_{e_1,n}(i) \cap \mathrm{neighborhood}_{e_2,n}(i) |
\]

\noindent\textbf{Spread} measures to what extent neighborhoods stay compact across embeddings.
Spread expresses how far a compact neighborhood expands in the other embedding. It is non-symmetric.% in terms of the two embeddings involved.
%In addition to neighborhood overlap, it offers additional insight into what happens to neighborhoods from one of the embeddings in the second embedding.
It complements overlap by measuring what happens to objects that do not remain in the near neighborhood in the other embedding.
We use three versions of spread.
The first one, singular spread, can help understand how stable or unstable neighborhood ranks remain across embeddings.
It supports tasks with a focus on analyzing fine-grained variations in the neighborhood representations, such as~\exhdtored.
It is defined as
\[
	spread_{e_1,e_2}(n, i) = rank_{e_2}^i(s_n^{e_1}(i))
\]
The neighborhood-max and neighborhood-median versions focus on the characterization of the maximum and average changes in the neighborhood, respectively.
Both versions help with different types of scenarios.
The neighborhood-max version is well suited for comparisons with less severe changes between neighborhoods, and help finding extreme cases, such as when comparing embedding versions on the same dataset (e.g., \exhdtored \exhypp and \exvecsz).
It is defined as
\[
	s\_max_{e_1,e_2}(n, i) = max( rank_{e_2}^i(s_1^{e_1}(i)), \ldots, rank_{e_2}^i(s_n^{e_1}(i)) )
\]
The neighborhood-median is more useful in cases where neighborhoods differ a lot by default, such as embeddings built on different datasets (e.g.,~\excorpora and~\exlanguages)
It is defined as
\[
	s\_med_{e_1,e_2}(n, i) = median( rank_{e_2}^i(s_1^{e_1}(i)), \ldots, rank_{e_2}^i(s_n^{e_1}(i)) )
\]

\subsection{Metrics of Distance}\label{sec:measures-distance}
This second category of metrics consider the distance relationships between objects.
Because distances are not directly comparable between embeddings (see \S\ref{sec:tasks_and_requirements}), they are computed and displayed for each embedding separately.
While the summary distributions of these metrics can be compared, the metrics are most often used to interpret differences identified with rank metrics.

\noindent\textbf{Average n-ball density} provides insight into how dense the local region around an object is.
By expressing this density as neighbor counts within embedding-specific radii that adapt to the average distances of each embedding, the resulting notion of density remains comparable across embeddings.
This metric helps in particular for higher dimensional data where distances tend to be less meaningful than densities, such as \exvecsz, \excorpora, and \exlanguages.
% It provides insight into one embedding at a time.
% Comparisons between embeddings are made by comparing visualizations of these distributions.
The metric is defined as the number of neighbors of an object within the distance of the average n-neighbors of the embedding
% \todo{wouldn't the metric make more sense if we normalize with the number of elements, ie. if it were a percentage?}
% \todo{Flo: I tried a version of that some time ago. As far as I remember, the reason I didn't like it was that interpretation and comparison was somehow more complicated. We could mention and discuss this more, but not sure if it's worth it.}
\[
	n\_density_e(n, i) = | \{ j | d_e(i, j)\leq mean_e(n) \} |
\]
with
\[
	mean_e(n) = \frac{\sum_{i\in E}d_e(i, s_n^{e}(i))}{|E|}
\]

\noindent\textbf{Neighbor Distance} is the distance of an item to its nearest neighbors.
This metric, in relation to the distribution of distances within the entire embedding helps gauge the significance of the neighborhood relationship.
We found this to be particularly helpful in lower dimensional embeddings, in which distances tend to be more tangible than densities, such as \exhdtored and~\exoverfit.
Like the previous metric, it is embedding-specific and comparisons are made by comparing distributions and single values across embeddings.
It is defined as
\[
	n\_dist_e(n, i) = d_e(i, s_e^n(i))
\]

\subsection{Pairwise Metrics}
This category provides a value for each pair of objects in the embeddings, unlike prior categories that provide a value per object.
% Because they consider many more values, these metrics are exclusively used for summary views.
% \todo{Flo: Not sure this statement is true; the other metrics are also only used for summary views, or am I missing something?}

\noindent\textbf{Pairwise Distance}, defined by $d_e$, is useful for interpreting object sets, particularly in higher-dimensional embeddings, relative to the entire embeddings (e.g., \exvecsz, \excorpora, and \exlanguages).
% For example, it can be helpful in gauging how central a set of objects is within the embedding.
% In addition, comparing shapes of the distribution provides insight into how the objects are spread out within two embeddings and whether there are differences.
Comparisons can be made between the distribution of these distances across embeddings, which provides insight into distributional differences of objects between the embedding.
In addition, comparing the distribution of a subset of objects to all others in an embedding can help understand how central the selected group of objects is on average within an embedding.
This metric is embedding-specific.
It is defined for a pair of objects, and yields a distribution for all possible object pairs in an embedding.

\noindent\textbf{Stress} is a metric that is used a lot and in various versions to measure the accuracy of dimensionality reductions compared to their source embedding (\exhdtored).
It measures the difference in distance between each pair of objects in the two embeddings.
Versions of this metric are sometimes also called \emph{strain}, and there is a whole family of dimensionality reduction methods that aim to minimize stress to create dimensionality reductions (see \S\ref{sec:related_work_embeddings}).
The version we use is based on the fraction of distances between a pair of objects in two embeddings
\[
	stress_{e_1,e_2}(i,j) = \log{\frac{d_{e_1}(i,j)}{d_{e_2}(i,j)}}
\]
Taking the $log$ has two effects: (1) It dampens the effect of relative large differences and reduces the range of the resulting scale used to represent them, and (2) it introduces a symmetry between differences in both embeddings with negative values for $d_{e_1}(i,j)<d_{e_2}(i,j)$ and positive values for $d_{e_1}(i,j)>d_{e_2}(i,j)$.
While stress is a good metric to gauge the overall fit between two embeddings, it overemphasizes distances between objects that are far away from each other in both embeddings, and for whom the absolute distances, depending on the type of embeddings, might not be that relevant.
Still, we found that it provides useful insights in our case studies, in particular when comparing the distribution of stress of a subset of instances to the entire distribution.


==> tex/mike-requirements.tex <==
We apply a framework for comparison~\cite{Gleicher2018} to provide an abstraction of the embedding comparison problem, to identify the key comparative challenges, and to suggest solution strategies.
First, we consider a range of example scenarios and abstract common tasks and task properties.
Then, we identify comparative challenges and connect them to a solution strategy. 
We focus on pairwise comparisons, as this is the simplest case.
%However, the examples below show a clear need for 
Multi-way comparisons should be addressed in future work.

\subsection{Example Scenarios}\label{sec:example_scenarios}
%\todo{Make sure abstract tasks get named in this section}
%Quantify the amount of meaningful difference between embeddings.
%Identify objects whose neighborhood changes contribute to the otherall change.
%Dissect the changes to an object's neighborhood to understand its causes.
%Re-connect the changes to an object to the broader context
%Connect changes in object neighborhoods to outcomes

We survey a set of representative scenarios of how embedding comparison may be used in practice.
These examples illustrate the potential utility of an embedding comparison tool, common tasks, and the diversity of challenges. We draw these examples from our experiences using embeddings as well some seen in the literature. 

% \textbf{beef up these examples to better support the points below}

\begin{enumerate}[label=\textbf{S\arabic*}]
% Maybe skip this example 
%\item \label{ex:2dr} A user may compare two runs of a dimensionality reduction algorithm with different random seeds (e.g., Section 3) in order to appreciate whether the differences between the outputs are significant or not. In these cases, minor changes (such as the random seed) may be expected to lead to similar structural properties yet very different global positions. 

\item \label{ex:hd2d} A designer may compare a high dimensional data set to a dimensionality reduction of it to 2D in order to check that a visual presentation of the dimensionality reduction adequately conveys the contents of the high-dimensional space.
They first check the overall amount of local structure preserved, and then investigate specific objects and object groups with substantial differences to see if these errors are acceptable.

\item \label{ex:hypp} A researcher may compare document embeddings from topic models built with different hyper-parameters to select a preferred model based on a subjective assessment of which provides better similarity recommendations.
They first survey the differences across the whole embedding to assess the amount of difference and identify documents with very different recommendations.
The differing neighborhoods for these documents can be assessed to select which is better.

\item \label{ex:vecsz} A developer may compare word vector embeddings built with different numbers of dimensions to determine the impacts of the increased storage costs of a larger space.
They may see how often words have different neighborhoods and what words are most affected by the differences.

\item \label{ex:absfull} A journal editor compares a document embedding from a topic model built from paper abstracts to one built from the full texts in order to assess whether the extra effort of obtaining the texts leads to better similarity measures that are used in identifying related documents.
They can check if the differences in embeddings lead to different clusterings of the documents, and whether documents that cluster differently are the ones most affected by the changes to the embedding.

\item \label{ex:overfit} A data scientist compares two supervised dimensionality reductions built from different amounts of training data to analyze potential overfitting of the learning algorithms.
After confirming the overall difference between the embeddings, they can identify specific objects with the most substantial change and determine if these are part of the changes to the training data.

\item \label{ex:corpora} A literature scholar compares word vector embeddings each built from a different collection of texts as a way to analyze the differences in word usages in the two corpora. 
This involves identifying words that stay constant or have dramatic changes, examining specific words to see how their neighborhoods change to assess whether this reflects change in meaning, and reconnecting specific words to the overall language by looking for groups and patterns of words that behave similarly.

\item \label{ex:languages} A linguist may compare word embeddings constructed from corpora in different languages in order to understand latent differences in word usage between the languages.
Here, the objects (words) in the different embeddings are not the same; however there is a known correspondence between some of them.

\end{enumerate}

%In many cases, 
Users currently address these kinds of tasks using either \emph{ad hoc} analysis or specialized tools. We use the list to abstract some key ideas that inspire a general tool for embedding comparison.

%% torsten's point is not completely addressed with the first sentence,
%% but it's the best I can do
% \textbf{TM: theses are all reasonable examples, however, two issues (1) while they seem straigh-forward to someone working in the field, it would be good if each scenario had a ref attached where this scenario is actually detailed. and (2) many of the state-of-the-art approaches does some of this numerically. It might be worthwhile to point out why/where a numerical characterization fails.}

\noindent\textbf{Global and local tasks:} Each scenario follows a similar pattern of tasks:
(1) generally assess the amount of difference between the embeddings,
(2) identify a set of objects whose neighborhoods differ in interesting ways,
(3) more closely assess the objects and their neighborhoods.
The changes in neighborhood may then be dissected to determine their cause, or re-connected to the overall embedding by finding other objects with similar behavior.
This list provides a core set of abstract tasks that our approach must address. Using the target/action task notation \cite{Munzner2014} as adapted for comparison \cite{Gleicher2018}, there are several common comparison targets: entire embeddings, collections of objects, and the neighborhoods of objects. Important actions include \emph{quantifying} the amount of difference, \emph{identifying} interesting sets and objects, \emph{dissecting specific differences to understand their cause}, and \emph{re-connecting} specific findings to the larger set or their impact on downstream uses.

%Some scenarios involve tasks that consider the entire embeddings, such as ``quantify the amount of meaningful difference.'' However, more commonly tasks involve identifying specific objects whose neighborhoods \todo{need to define neighborhood} compare in interesting ways (e.g., having very similar or different sets of neighbors in the two embedding). \textbf{Why is example finding so useful}. 

The ability to identify and analyze the changes in neighborhoods is central to all comparison scenarios we have considered.
This ability is particularly important in the common cases where there is no ground truth so assessment requires some degree of subjectivity.
For example, in assessing the differences between two topic models, if a document has very different neighbors, an expert may want to evaluate if one set is preferable to the other, or whether the document can be disregarded as an outlier so the differing performance is not important.
Identifying specific objects is often more interpretable to a user than more abstract relationships between objects, and provides a connection to the semantics of the embedding.
For example, in a word embedding, the user most likely understands the objects (words) and has considerable background knowledge to interpret how words behave.

%\textbf{do we want to formally state abstract tasks in target/action notation?}
% \todo{Flo: I am not sure how helpful that is. It might help to motivate the metrics in section 5, but it also gets complicated quickly. I tried to put the above list of task patterns into the verb-object form.}
%\todo{TM: ideally yes}

% When embeddings are constructed, there is rarely a ground truth so assessment requires some degree of subjectivity. In such cases, the ability to identify and examine specific differences is particularly important. 

% When specific objects are identified, two types of task emerge. Some tasks dissect the object neighborhood comparison, asking ``why'' they are similar or different. Such questions are best answered by tools that can explore the details of the embeddings. Other tasks involve gaining context for the specific comparison, for example to understand if the difference is unique, or to identify other objects with similar properties. Similarly, changes to object neighborhoods may be connected to downstream outcomes such as clustering results.

\noindent\textbf{Understanding models vs. understanding data:}
Users have two types of goals.
Some scenarios (\exhdtored, \exhypp, \exvecsz) involve comparing different embeddings of the same data in order to understand the differences between models.
%For example, the user may compare embeddings built with different algorithms or parameters.
In contrast, other scenarios (\excorpora, \exlanguages) involve comparison of embeddings built from different data
as a way to compare the underlying data sets.
% Such scenarios seek to understand the relationships between the initial data sets used.

When the same data is used to construct the embeddings, the set of objects in the embeddings will be the same.
However, with different data, embeddings may have different objects (\exlanguages).
In this work, we focus on comparisons with overlapping sets of objects; for comparisons with different objects we rely on correspondences between embeddings (e.g., matching words between languages).

\noindent\textbf{Different uses of embeddings:}
The scenarios make use of the similarity and difference information in embeddings in different ways.
Some scenarios seek to identify similar objects (\exabsfull), while others use this information for other processes such as clustering or nearest-neighbor classification (\exoverfit), or creating 2D models for visual presentation that place similar objects close together (\exhdtored).
All of these uses of embeddings focus on the similarity information in the embedding; the points assigned to objects are less important than the distances between objects.

In many cases, such as word vector embeddings or t-SNE dimensionality reduction, the embedding spaces are abstract, i.e., the dimensions have no meaning other than providing a space where relationships between objects hold.
In some cases, such as topic models, the dimensions may have some semantic meaning.
For such scenarios, global positions may be important.
These can be addressed with standard high-dimensional analysis techniques.

\noindent\textbf{Differences in embedding spaces:}
In many cases, the embeddings to compare are in different spaces.
The spaces may differ by numbers of dimensions, or have very different scalings.
Such differences preclude direct comparison of object coordinates, or even of the distances between objects.
Therefore, we focus on using distance ranks (i.e., orderings of closeness) as such measurements are invariant to dimensionality and scaling; two objects can be nearest neighbors in very different spaces.
However, the distance values may be important in understanding the causes of distance rankings.
For example, a small change in an object's distance may cause a large change in its rank if there are many objects with similar distances.
We must thus provide both rank- and distance- based metrics and allow for using the two types together.

\subsection{Challenges and Solution Strategy}
\label{sec:strategies}
Gleicher~\cite{Gleicher2018} identifies three categories of comparative challenges.
%In this paper, we restrict ourselves to pairwaise comparison, which allows us to avoid 
This paper focused on pairwise comparison, avoiding
the challenge of large numbers of targets for comparison.
%\todo{Flo: As I see it, there is a second interpretation (or maybe level) to this: Numbers of targets is potentially huge (because embedding has many objects), and objects may be complex (depending on what objects are embedded).}
This leaves the challenges of large targets (embeddings may have large numbers of objects) and complex relationships (each object's local neighborhood may change in many ways).

\noindent\textbf{Challenges of Complexity:}
The complexity of embedding comparison stems from the fact that the important similarities (whether objects are close together) may be obscured by other differences (their positions in space may be different).
To manage this complexity, we focus our attention on the objects and their neighborhoods, including the distances between objects in these neighborhoods.

We break the comparison of embeddings into the comparison of the neighborhoods of each object in the embedding.
% \todo{Flo: This gives rise to new challenge of scale.}
Given a pair of neighborhoods corresponding to an object in a pair of embeddings, we can define a number of metrics that capture the degree of difference in the distance relationships.
More global comparisons consider the distributions of these per-object comparisons.
\S\ref{sec:measures} considers a set of metrics for comparing neighborhoods, and \S\ref{sec:designs} introduces a set of views for summarizing distributions of the metrics for global assessment, as well as detail views for examining specific objects and their neighborhoods.

\noindent\textbf{Challenges of Scale:} To address the challenges of scale, we use all three scalability strategies~\cite{Gleicher2018,alpersummarize}.
First, we use \emph{summary} views that aggregate per-neighborhood metrics across the embeddings.
These views show the distributions of the various metrics, and allow the user to both have an overall sense of the amount of similarities and differences, but also to identify sets of objects that have interesting values of the metrics for further exploration.
These interesting subsets may be \emph{selected} to focus analysis on a more manageable portion of the object collection.
Our approach provides mechanisms for creating complex selections by combining groups seen in summary views, and provides views that allow details of moderate sized groups to be examined.
\emph{Scanning} in these mezzo-views is used to identify specific objects to examine details.

==> tex/motivation.tex <==
% To motivate the need for embedding comparison and illustrate the challenges in performing it, 
To illustrate the challenges of embedding comparison and our approach, 
we consider a simple example: reducing a 10-dimensional data set to 2 dimensions so that it can be presented visually.
Specifically, we begin with a 10-dimensional topic model trained on papers published at the IEEE VIS conference~\cite{Isenberg2017}, from the years 1990--2016.
% The topic model places the documents into the 10-dimensional space such that similar documents are close together.
We seek a reduction of the 10-dimensional space to 2 dimensions that preserves close neighbors so that objects that are close visually are similar documents.
To perform the dimensionality reduction, we use the t-SNE algorithm~\cite{Maaten2008} that attempts to preserve the near neighbors of objects.
% The result of t-SNE is an embedding of the 10-dimensional objects into 2-dimensional space.
%If we run the t-SNE algorithm twice on the same data, we get very different positions for the points overall, because each execution uses a different random seed.
Running the t-SNE algorithm twice on the same data provides different positions for the points because each execution uses a different random seed; 
% as illustrated in FIGURE\todo{add figure} because each execution uses a different random seed.
t-SNE preserves distance relationships between points, and absolute positions may be arbitrary.
We can see this effect in Figure~\ref{fig:scatter_ex1}, which shows the results of the two t-SNE runs.
The colored circles show corresponding clusters in both embeddings which remain together despite the overall changes in point positions.

Our expectation is that each point has similar neighbors in each embedding:
for any point $i$ in the embeddings, the set of points close to $i$ in one embedding should contain the same points as the set for the other embedding.
The \emph{overlap} metric, defined in \S\ref{sec:measures}, measures this similarity.
% To measure this similarity we use a metric called \emph{overlap} that measures for each object in the embedding how many of its $n$-nearest neighbors in the first embeddings are also in its $n$-nearest neighbors of the second embedding.
It counts the number of neighbors shared among the closest $n$ neighbors for each object.
For a given value of $n$, a pair of embeddings has a distribution of values of overlap for each object.
The distribution can be summarized in a histogram. 
For example, Figure~\ref{fig:overlap_buildup1_ex1} shows the distribution of overlap values for $n=1,$ revealing that most points have $overlap_1=1,$ meaning that they share the same nearest neighbor. 
% For example, for $n=1,$ the embeddings have 651 objects with overlap of 1 (meaning the nearest neighbor is the same in both embeddings), and 216 objects with overlap of 0.
% FIGURE\todo{add figure} shows the distribution of this metric as a histogram for values of $n$ from 1 to 5.
%Figure~\ref{ fig:overlap_buildup } shows the distribution of this metric for neighborhoods of size 1 (Figure~\ref{fig:overlap_buildup1_ex1}), and sizes 1-5 with two different encodings (Figure~\ref{fig:overlap_buildup2_ex1} and~\ref{fig:overlap_buildup3_ex1}).
%In Figure~\ref{fig:overlap_buildup1_ex1}, we can see that the majority of object keeps its nearest neighbor.
Figure~\ref{fig:overlap_buildup2_ex1} shows histograms for n between 1 and 5, indicating, for example that most points have 4 or 5 of their 5 nearest neighbors in common. 
Figure~\ref{fig:overlap_buildup3_ex1} shows this same data using a color encoding rather than a bar chart. We prefer the color encoding because it will scale well to larger numbers of neighborhoods (e.g., Figure~\ref{fig:overlap_ex1}), and provides a full size box even for small values which makes it easier to select.

% Tooltips for the bars reveal that there are 651 overlaps with size 1 (top bar), and 251 overlaps with size 0 (bottom bar).
% Looking at the top right of Figure~\ref{fig:overlap_buildup3_ex1}, we can see that the majority of objects have a 5-overlap of 4 or 5, i.e., 4 or 5 of their 5 nearest neighbors are common across embeddings.
% The legend for the color encoding is shown in top of the plot.
%It normalizes count values per column

%The color encoding in Figure~\ref{fig:overlap_buildup3_ex1} allows us to scale to higher neighborhood sizes than with histograms.
The \emph{overlap view} provides an assessment of the degree of similarity between the embeddings.
Figure~\ref{fig:overlap_ex1} shows the overlap for values of $n$ up to 50.
The dark blue rectangles near the top right, for example, show us that large numbers of objects have 48 or 49 of their neighbors in common, confirming that most objects have very similar sets of neighbors.
However, there are exceptions: the green box (highlighted with a red square) near the right edge shows that there are several (hovering reveals the exact number to be 16) objects that only share 15 out of 50 neighbors. 

The overlap view also serves as an input mechanism: clicking on any box selects its content.
Conversely, any box (or other display element) that contains selected items is shown with a red border.
Therefore, selecting the green box at the right of Figure~\ref{fig:overlap_ex1} not only highlights that box, but highlights other boxes that contain the members of the selected box.
These points are also highlighted in other views (such as Figure~\ref{fig:scatter_ex1}).

\begin{figure}
	\centering
	\begin{subfigure}[t]{.25in}
		\includegraphics[height=1.5in]{pictures/overlap_buildup_1.png}
		\subcaption{\label{fig:overlap_buildup1_ex1}}
	\end{subfigure}
	\qquad
	\begin{subfigure}[t]{1.2in}
		\includegraphics[height=1.5in]{pictures/overlap_buildup_2.png}
		\subcaption{ \label{fig:overlap_buildup2_ex1}}
	\end{subfigure}
	\qquad
	\begin{subfigure}[t]{1.2in}
		\includegraphics[height=1.5in]{pictures/overlap_buildup_3.png}
		\subcaption{\label{fig:overlap_buildup3_ex1}}
	\end{subfigure}
	\\
	\begin{subfigure}[t]{3in}
		\includegraphics[width=\columnwidth]{pictures/overlap_ex1_hilite.png}
		\subcaption{\label{fig:overlap_ex1}}
	\end{subfigure}
	\caption{ Three versions of the \emph{neighborhood overlap} summary view.
					It shows the distribution of \emph{overlap} between neighbors of the same object across two embeddings.
					(a) shows distribution for neighborhoods of size one as a (vertical) histogram,
				    (b) shows the distributions for neighborhoods of sizes 1-5 with multiple columns,
			    	(c) shows the same distribution with a color encoding for the count numbers instead of bar heights,
			    	(d) shows the distribution for sizes 1-50; the highlighted boxes (red border) contain selected objects.
		    		The color legend for plot (c) and (d) is shown on top.
	    			Count values are normalized per column.
    				\label{ fig:overlap_buildup } }
\end{figure}

\begin{figure*}
	\centering
	\includegraphics[width=\textwidth]{pictures/scatter_ex1_marked.png}
	\caption{ Scatterplot view of both t-SNE embeddings of the visualization papers topic model.
				   The highlighted (red) documents were selected %, because they %appeared as outliers with particularly low overlap in their 50-neighborhood in the overlap view (see
				   by selecting items with 15 overlaps in their 50-neighborhood in Figure~\ref{fig:overlap_ex1}).
			   	   We can see that they are in different positions within the spatialization.
		   	   	   In the one on the left, the cluster seems to be an outlier, far away from other documents, while on the right, the same cluster appears in the vicinity of a larger, bigger one.
	   	   	   	   The colored circles show other clusters in both plots. }
	\label{fig:scatter_ex1}
\end{figure*}


% From Figure~\ref{fig:overlap_ex1} we can see that the two embeddings consistently have similar neighbors.
% We are interested in whether they introduce any qualitative differences to the embeddings, and we start looking at them in more detail.
% One of the bins we come across during our exploration contains an entire cluster in both embeddings.

Selecting a group of objects allows them to be explored in detail in other views. For example, we can see in the \emph{scatterplot view} (Figure~\ref{fig:scatter_ex1}) that the group is a cluster of points that remains close together, despite moving in position. We can use the \emph{selection list} view (not shown, but discussed in \S\ref{sec:design}) to identify these points as corresponding to documents with ``uncertainty'' in their title.

%The selected box in column 50 (red border) seems to be an outlier.
%In the scatterplot view (Figure~\ref{fig:scatter_ex1}), we can see that this is a cluster with 16 documents in both embeddings (selected documents are colored red).
%In the left one, the cluster is in a region by its own, while in the right embedding it is connected to an additional small cluster (green circle) in the vicinity of a much larger one to its upper right (purple circle).
%Viewing the titles of the documents in the selected cluster, we learn that it exclusively contains papers that examine and introduce visualization methods for uncertainty (14 of the 15 members of the cluster have the word \emph{uncertainty} in their title).
%Interestingly, the small cluster (green) contains 5 documents about flow visualization, and all of them deal with some aspect of uncertainty.
%Finally, we inspect the large cluster (purple) and find that it exclusively contains flow visualization papers.
%We find that the two clusters have corresponding ones in the other t-SNE embedding that are close to each other, but far from our original cluster (cluster correspondences are highlighted with the same color in Figure~\ref{fig:scatter_ex1}).

Further exploration may use other views that summarize different metrics. For example, Figure~\ref{fig:spread_ex1} shows a \emph{spread view} that summarizes the spread metric defined in \S\ref{sec:measures-rank}. This view shows us that despite the high overlap seen in Figure~\ref{fig:overlap_ex1}, most neighborhoods of size 25 have at least one object that moves far away. 

%Figure~\ref{fig:spread_ex1} helps us put this phenomenon into a global context.
%It show the distribution of neighborhood-max spread for neighborhood sizes 1-25 (along the horizontal axis).
%The neighborhood-max spread for the neighborhood of size $n$ for object $i$ in one embedding is the maximum size of the neighborhood of object $i$ in the second embedding that contains all $n$ neighbors of $i$ from the first embedding.
%It is thus a measure for how compact neighborhoods stay between two embeddings.
%Each of the columns in Figure~\ref{fig:spread_ex1} shows the distributions of those neighborhood sizes from the left t-SNE embedding to the right one, with colored boxes for each neighborhood size in the second embedding, up to size 100.
%The plot uses the same color coding for the boxes as before.
%The boxes at position 100 contain all neighborhoods of size 100 and beyond in the second embedding.
%The metric is explained in detail in \S\ref{sec:measures}, and the visual design in \S\ref{sec:designs}.

%We can see that, between our two embeddings, neighborhoods tend to stay relatively compact until around size 10 (most of the blue and green boxes in that column are below 15), with a rising variance roughly between size 10 and 18.
%Beyond 18, things diverge quickly.
%Our selected cluster has size 15, and falls right into this high-variance range (see red highlights in Figure~\ref{fig:spread_ex1}).
%This suggests that what we have looked at is an inconsistency introduced by the t-SNE algorithm with the particular  parameterization.
%Since we want small clusters to stay close to other, similar documents within the 2D embedding, we can now start to explore different parameterizations and dimensionality reduction methods.
%Through evaluation by comparison, we can assess whether they result in better, more consistent results for the placement of such clusters.

% \todo{this is not a motivating example, this is already a use case. I would NOT put a use case that early without explaining the visual encodings and metric! A motivating example stops with the first paragraph. The end of the paragraph should be a number of questions that are open.}

\begin{figure}
	\centering
	\includegraphics[width=\columnwidth]{pictures/spread_ex1.png}
	\caption{ Spread view shows diversion of neighborhoods.
				     The horizontal axis shows neighborhood size (for the left t-SNE embedding).
				     Each column represents a neighborhood size of $n$.
				     For each, the vertical axis shows the distribution of neighborhood sizes in the right embedding that contains the entire neighborhood of size $n$. The top row indicates that the neighbors are not contained in the nearest 100.
				     The view tells us how compact neighborhoods generally stay across the two embeddings.
			   	     Bins with a red outline contain members of the selected cluster (see Figure~\ref{fig:scatter_ex1}). 
		   	     }
	\label{fig:spread_ex1}
\end{figure}


==> tex/require.tex <==
In this section, we derive a set of tasks and requirements that form the basis for the discussion of our approach.

\subsection{Analysis Scenarios and Tasks}
We collected a set of practical scenarios for comparing embeddings according to a range of different aspects.
Those scenarios are either important to domain experts that use embeddings to analyze data, or data scientists creating, evaluating, and improving embeddings methods and the general process of creating them.
Generally, the types of scenarios that we aim at supporting can be categorized along 5 dimensions.
These dimensions all have an influence on the types of measures, visualizations, and interactions needed to comprehensively support the scenario.
In the following we list the dimensions and then discuss concrete examples for them.

\noindent \textbf{Compare data or embedding}
There are two different types of goals that users may have as a motivation for comparing embeddings: either gain insight into the embedding itself, or into the source dataset used to build it.
% The former category includes scenarios in which users aim to understand the influence of parameter settings on the embedding, or differences in how various algorithms model the data.
An example for the former is \textbf{(1)} \textit{Comparing and understanding two different dimensionality reductions of a high-dimensional data set}, for which we have seen an example in \S\ref{sec:motivation},
while \textbf{(2)} \textit{Comparing two different versions of a language through word embeddings} is an example for the latter type.

\noindent \textbf{Abstractness of objects}
The tangibility of the objects influences the type of analysis that users may want to do with an embedding, and what prior knowledge and hypotheses they have about the objects.
On the one end of this dimension, we have very concrete objects, such as text documents.
An example would be \textbf{(3)} \textit{Comparing RCA models built on different training and tests splits of a set of English plays categorized into different categories}.
A \textbf{(4)} \textit{Comparison of character n-gram embeddings with different parameters} would be on the other end of the spectrum.\todo{cite fasttext here?}

\noindent \textbf{Abstractness of dimensions}
% In addition to how abstract the embedded objects are, it is also relevant how easily interpretable the single dimensions of the embedding are.
An example for a scenario involving embeddings with meaningful and interpretable dimensions is \textbf{(5)} \textit{Comparing different topic models for a set of documents}, where topics form the dimensions of the embedding space.
% On the other hand, \textbf{(6)} \textit{Comparing a word embedding created with two different algorithms} is an example of a comparison of two embeddings in which the dimensions have no meaning, and only vector relations encode information.
Since the dimensions are a property of one embedding, comparisons between heterogeneous embeddings are possible.
An example for this is \textbf{(6)} \textit{Comparing a set of documents embedded into a topic space to a 2D tSNE reduction}.

\noindent \textbf{Scale of dimensionality}
The embedding pairs to compare can have differences in their dimensionality, from hundreds of thousands of dimensions, e.g., for raw vocabulary vectors to represent documents, to two dimensions for a dimensionality reduction created for visualizing a data set.
The most challenging scenarios to support are those in which the dimensionality between the embeddings to compare is significantly different.
For example, \textbf{(7)} \textit{Comparing a 300D word embedding to its 2D dimensionality reduction}.
\todo{Overview visualizations must scale to large differences in dimensionality; discuss in requirements!!}

\noindent \textbf{Scale of number of objects}
Embeddings to compare can have a large range of different sizes.
From embeddings that contain about a dozen object, such as \textbf{(8)} \textit{Comparing topic models of Shakespeare's plays}, to potentially millions of objects, such as \textbf{(9)} \textit{Comparing word embeddings created with different parameterizations}.
\todo{Overview vis must be visually scalable to a potentially large number of object; filter are important to drill down to single examples.}

\subsection{Requirements}\label{sec:requirements}
Based on this set of concrete tasks, we now describe the challenges and design requirements that the approach must fulfill.

\noindent \textbf{R1: Scalable Overviews}
Analyses can either start with a concrete hypothesis about a set of objects, or a very general notion of how the embeddings might differ.
This is influenced by the kinds of insights users want to gain (e.g., \textbf{task 1} versus \textbf{task 2}), and how concrete the embedded objects are (e.g., \textbf{task 3} versus \textbf{task 4}).
For the second type of scenarios, users need an entry point into the analysis that helps them identify interesting phenomena and sets of objects for closer inspection.
In addition, providing a global view of existing differences and similarities between the embeddings helps develop and solidify hypotheses about embeddings and source data that can later be tested.
The visualizations that provide users with such an overview must be visually scalable to potentially large numbers of objects, and work for embeddings that are heterogeneous in terms of dimensionality (\textbf{task 7}) and object distribution.\todo{mention things like scale, rotation, ... invariance?}
%As a basis for the overview visualization, distributions of relevant object properties within and between two embeddings are needed.
%For this, a set of metrics to quantify object-level differences between embedding spaces can serve as a basis.
%POTENTIALLY MOVE TO METRICS SECTION
%To extract and summarize relevant object properties, numeric measures (or degree-of-interest functions) are needed.
%Those can either quantify and summarize object properties, or they are comparative and directly quantify differences between object properties within embeddings.
%Depending on which type of measure a visualization is based on, it either directly encodes differences between embeddings, or juxtaposes summary visualizations of properties that facilitate visual comparison.
%In addition, in case such information is available for the objects in an embeddings, summarizations of relevant meta data into informative visual representations may provide additional important insights into the differences between embeddings.
%Examples include publications years of documents, or frequency information for words in word embeddings.
%\todo{How do we support / handle large differences in dimensionality in the overview visualizations? Explain!!}

\noindent \textbf{R2: Everything in Context}
%In addition to an entry point into analysis and a way of helping to generate hypotheses,
Overviews also provide a point of reference during analysis.
For this, single objects and aggregated groups should be shown within the distributions depicted in the overview visualizations, as well as in any local view.
%In addition, objects should be cross-linked and highlighted across local views (see \textbf{R5}).
This supports sense making~\cite{Klein2007} by providing additional information about data fragments to help confirm or reject hypotheses.
%An object set's context comprises its distribution within all views such that users can identify combinations of properties that render them interesting in some way.
In addition, meta data of an object (e.g., authors, title, and abstract of scientific papers) should be linked to the objects.
This helps interpret single objects, and groups through representative examples, in particular for more tangible objects (e.g., \textbf{task 3}).
For embeddings that have interpretable dimensions, the affinity of objects to different dimensions can be of additional relevance (\textbf{task 5 and 6}).
%An example for such a phenomenon would be a group of few objects that is grouped together closely (are comparatively close to their nearest neighbors) in a generally very low density region of an embedding, far off from other objects.
%In addition, context from the original data set, such as meta data of the object (e.g., authors, title, and abstract of scientific papers) show be provided if available for an embedding.
%It can help with the interpretation and correlation of single objects, and help explain the contents of groups by picking representative examples.

\noindent \textbf{R3: Guidance for Drill-Down}
One aspect of assuring scalability with a large number of objects (\textbf{task 9}) is to provide support for selecting representative objects that help generate as well as confirm or reject hypotheses.
Strategies for picking examples that should all be supported are:
(1) objects that differ most or least across embeddings, (2) objects that are most prominent within a group, by some measure of prominence, to understand the gist of a group, and (3) central and corner cases to illustrate the composition of a group.
In addition, grouping objects by similarity according to various criteria in both embeddings, and comparing those groupings, may help uncover structure and generate additional hypotheses about the spaces, in particular for abstract objects with little meta data (\textbf{task 4}).
% Users should be supported with all three strategies to drill down to single examples to ground their analyses in.
% explain later: we satisfy these requirements by design of selection management, sorting (in list views) and filtering, visual representations in 2D, clustering (overlapping and non-overlapping subsets of clusters)

\noindent \textbf{R4: Comprehensive Filters}
Filters are one aspect of providing support for drill-down operations.
They are also essential to support scenarios in which users starts with concrete hypotheses about specific objects (e.g., \textbf{task 3}).
The design should support identifying single objects within large embeddings, for example, through directly searching for a document title.
This is particularly relevant for smaller datasets (e.g., \textbf{task 9}), but may also be important for larger ones, in particular when the analysis goal is learning about the source dataset (\textbf{task 2}).
Filtering groups of objects should also be possible, either based on meta data, or on distributional properties and similarities within the embeddings.
For this, direct interaction with the overview visualizations should be possible to interactively modify filter criteria.
% SOME ADDITIONAL THOUGHTS:
% again, we support this through our advanced selections, free text search, and support for sorting
% filters for non-concrect objects: doing a clustering and comparing them scross embeddings to come up with ideas / good sets to compare
% filtering based on properties within the embeddings: directly interacting and selecting from the overview visualizations is possible
% selection by distributional properties and similarities within the embedding is another motivation for metrics and corresponding visualizations

\noindent \textbf{R5: Local Comparisons}
Finally, support for analyzing and comparing examples locally help users learn about details of a particular pair or small set of objects.
This is particularly vital for tasks that involve small datasets or concrete objects (\textbf{tasks 3 and 8}), and an important aspect of all previously listed scenarios.
Local views should cover all the aspects covered by the overviews, and provide links back to the global context of an example to connect it back to the larger analysis scenario.
% As for the overview visualizations, context should also be preserved in the local views of selected phenomena.
% This includes links and connections to other objects that are part of the display, e.g., local neighbors of a particular object.
% To facilitate users with grounding higher level phenomena from the overview visualizations in local examples, the larger context of the selected objects should be preserved and accessible during analysis.
% This way, examples can be easily traced back to their global positions, and new neighboring or otherwise similar examples can be added to the local view that help to corroborate or reject hypotheses during analysis.

==> tex/use_case_absVfull.tex <==
Models of scientific paper collections may be built from either the metadata (e.g., abstracts) or the full texts of each paper.
To explore this choice we collected a corpus of about 1500 papers from recent visualization conferences and built one document model using the paper abstracts and a second using the full texts.
Both models were generated using NMF (see \S\ref{sec:related_work_embeddings}), with 10 topics each.
This is a variation of the \exhypp scenario (\S\ref{sec:example_scenarios}), where we compare topic models based on different versions of the source dataset.

We start our analysis with the \emph{overlap view} to  assess the similarity between embeddings.
The overlaps tend to be low, in particular for smaller neighborhoods.
% most of the neighborhoods have an overlap of less than 50\%.
% In particular, smaller neighborhoods tend to have very little overlap.
To interpret this, we examine the \emph{neighborhood distance view} to check that the near neighbors of objects are close.
%(Figure~\ref{fig:ndistance_ex2}).
We see that for any given neighborhood size, the neighborhoods in the full-text embedding are smaller, suggesting that the full-text embedding is able to use the additional information to bring similar documents closer. 

%\begin{figure}
%	\centering
%	\includegraphics[width=\columnwidth]{pictures/fta_interlaced.png}
%	\caption{Neighborhood distance view showing the distribution of distances in both embeddings for neighbors 1 to 10.
%				   The full text model is on the left, and the abstract model is on the right.
%			   	   We can see that neighborhoods in the abstract model are generally less dense then the neighborhoods based on the full texts.
%		   	       }
%	\label{fig:ndistance_ex2}
%\end{figure}

To explore documents that do have agreement, we use the \emph{overlap} view to select documents that share 42 or more of their 50 nearest neighbors.
Using the \emph{selection list view}, we observe that 22 of these documents have the word \emph{tensor} in their title.
We reduce the selection to these documents, and view them in context with the \emph{scatterplot} view with t-SNE reduction.
% and topic pseudo-documents (\S\ref{sec:design-context}).
The documents form a tight cluster in both embeddings.
By using the \emph{scatterplot view}, we are able to identify other clusters that cover \emph{flow visualization} and other topics.
However, the \emph{scatterplot view} together with \emph{neighborhood wall view} also reveals that not all publications appear in similar clusters in both embeddings.
Some of them have entirely different neighborhoods with no overlap at all, even for high neighborhood ranks.
We then analyze the vicinities and clusters of these documents in both embeddings, and the abstracts and contents of some of the publications we identify.
The results suggest that the abstracts spend a greater proportion of their words describing the applications, while the papers are more focused on the methods.
This trend causes a difference in the models built from both data sources.


%We use the scatterplot of full texts to extend the selection with nearby documents.
%Examination of the details of this set reveals that the papers all relate to tensor visualization.
%The set forms a cluster in both embeddings, suggesting a topic similarly captured by paper abstracts and texts.
%However, there are a few outliers in the set: documents in the cluster in the full text embedding, but far away in the abstract embedding.
%Examining the details of one reveals a paper whose contents focus on methods, while the abstract focuses on its flow visualization application.

%To explore this phenomenon in detail,
%we return to the tensor selection set and extend it by documents that are close in the abstracts view.
%We examine this selection in the \emph{neighborhood wall} view (Figure~\ref{fig:wall_ex2}).
%This view confirms that most documents have their neighbors in the abstracts embedding stay close in the full-text embeddings and a few have their neighbors go farther away.
%Examination shows that these papers use the word tensor extensively in the abstract, even the content focuses on other aspects.

%\begin{figure}
%	\centering
%	\includegraphics[width=\columnwidth]{pictures/use_case_wall.png}
%	\caption{ Neighborhood wall for the selection in the abstract embedding.
%				   Columns represent documents in the set, rows are their ranked neighbors (the top row is the nearest).
%				   The position encoding represent neighbors in the abstract model, while the color encodes the rank of these neighbors in the full-text model.
%			       We can see that documents on the right have their near neighbors move far away. }
%	\label{fig:wall_ex2}
%\end{figure}

%Because both spaces have the same dimensionality and scale, comparing distances directly is meaningful, but may still be distorted by a scaling factor. \todo{How big is the distortion? Its still meaningful?}

%\todo{what is the task/goal of this usecase?}
%We start our analysis with the \emph{overlap view} to  assess the similarity between embeddings. The overlaps tend to be low,
%most of the neighborhoods have an overlap of less than 50\%.
%In particular, smaller neighborhoods tend to have very little overlap. \todo{should this be explained how we can see this?}
%To interpret this, we examine the \emph{neighborhood distance} view to check that the near neighbors of objects are close (Figure~\ref{fig:ndistance_ex2}). We see that for any given neighborhood size, the neighborhoods in the full-text embedding are smaller, suggesting that the full-text embedding is able to use its additional information to bring similar documents close. \todo{why is this the answer to denser neighborhoods in the fulltext embedding?}

%\begin{figure}
%	\centering
%	\includegraphics[width=\columnwidth]{pictures/fta_interlaced.png}
%	\caption{Neighborhood distance view showing the distribution of distances in both embeddings for neighbors 1 to 10.
%				   The full text model is on the left, and the abstract model is on the right.
%			   	   We can see that neighborhoods in the abstract model are generally less dense then the neighborhoods based on the full texts.
%		   	       }
%	\label{fig:ndistance_ex2}
%\end{figure}

%To explore documents that do have agreement, we use the \emph{overlap} view to select documents that share 42 or more of their 50 nearest neighbors between embeddings by combing boxes in the upper right. Using the \emph{selection list} view, we observe that 22 of these documents have the word \emph{tensor} in their title.
%We reduce the selection to these documents, and view them in context with the \emph{scatterplot} view with t-SNE reduction and topic pseudo-documents (\S\ref{sec:design-context}). The documents form a tight cluster near a topic in both embeddings. We use the scatterplot of full texts to extend the selection with nearby documents. Examination of the details of this set reveals that the papers all relate to tensor visualization. The set forms a cluster in both embeddings, suggesting a topic similarly captured by paper abstracts and texts. However, there are a few outliers in the set: documents in the cluster in the full text embedding, but far away in the abstract embedding. Examining the details of one reveals a paper whose contents focus on methods, while the abstract focuses on its flow visualization application.

%To explore this phenomenon in detail,
%we return to the tensor selection set and extend it by documents that are close in the abstracts view.
%We examine this selection in the \emph{neighborhood wall} view (Figure~\ref{fig:wall_ex2}). This view confirms that most documents have their neighbors in the abstracts embedding stay close in the full-text embeddings and a few have their neighbors go farther away. Examination shows that these papers use the word tensor extensively in the abstract, even the content focuses on other aspects.

%\begin{figure}
%	\centering
%	\includegraphics[width=\columnwidth]{pictures/use_case_wall.png}
%	\caption{ Neighborhood wall for the selection in the abstract embedding.
%				   Columns represent documents in the set, rows are their ranked neighbors (the top row is the nearest).
%				   The position encoding represent neighbors in the abstract model, while the color encodes the rank of these neighbors in the full-text model.
%			       We can see that documents on the right have their near neighbors move far away. }
%	\label{fig:wall_ex2}
%\end{figure}

%To find further evidence of such abstract / full-text misalignment, we look for examples where documents have very different neighborhoods.
%Selecing documents that have no agreement (0 out of 50 neighbors) in the \emph{overlap} view, the selection list shows many papers from medical or chemistry domains. In the \emph{scatterplot} view, we see that many papers are concentrated near a pseudo-document in the upper right corner.

%To further explore this phenomenon, use the scatterplot view to select papers near a psuedo-document for a topic in the full-text embedding  (Figure~\ref{fig:topics-scatter}).
%The view shows these documents are scattered in the abstracts embedding.
%Examining these papers in the \emph{selection list} view shows them to be papers about GPU-based methods.
%This suggests that the abstracts spend a greater proportion of their words describing the applications, while the papers are more focused on the methods.
%This trend causes a difference in the models built from the data sources.

%\begin{figure}
%	\centering
%	\includegraphics[width=\columnwidth]{pictures/scatter-w-topics-GPU.png}
%	\caption{Scatterplot view of two NMF models (left: full texts, right: abstracts). The 10-dimensional models are reduced to 2D by t-SNE, with pseudo-documents used to place topics (denoted by large red circles). A selected cluster in full-text embedding (red, upper right) scatter between topics in the abstracts embedding. }
%	\label{fig:topics-scatter}
%\end{figure}

%To further explore this phenomenon, use the scatterplot view to select papers near a psuedo-document for a topic in the full-text embedding  (Figure~\ref{fig:topics-scatter}). The view show these documents are scattered in the abstracts embedding. Examining these papers in the \emph{selection list} view shows them to be papers about GPU-based methods. This suggests that the abstracts spend a greater proportion of their words describing the applications, while the papers are more focused on the methods. This trend causes a difference in the models built from the data sources.
%\begin{figure}
%	\centering
%	\includegraphics[width=\columnwidth]{pictures/scatter-w-topics-GPU.png}
%	\caption{Scatterplot view of two NMF models (left: full texts, right: abstracts). The 10-dimensional models are reduced to 2D by t-SNE, with pseudo-documents used to place topics (denoted by large red circles). A selected cluster in full-text embedding (red, upper right) scatter between topics in the abstracts embedding. }
%	\label{fig:topics-scatter}
%\end{figure}


==> tex/use_case_eebo.tex <==
We are collaborating with literary linguists who are interested in how the English language has changed over the centuries.
To explore these changes, we have constructed word vector embeddings from two different corpora: a historic corpus consisting of over 50,000 books published between 1475 to 1700 from the Early English Books Online (EEBO) collection as transcribed by the Text Creation Partnership (TCP)~\cite{eebo-tcp} and a modern corpus built from the English language Wikipedia.
This is a variation of scenario \excorpora (\S\ref{sec:example_scenarios}).
We expect that changes in word meanings between the two eras would be reflected in the differences between their respective word vector embeddings.
For the experiments described here, we built the embeddings using GloVe with 300 dimensions, a window size of 15, and a minimum token count of 5.

We begin with the \emph{overlap view}.
Most words have low overlap.
Selecting the boxes with more then 50 percent overlap in the 50-neighborhood column we create a selection with 116 words.
Examining the list in \emph{selection list view} reveals that many of the words are function words and number words.
This is not surprising as these words have not changed in usage or meaning over the centuries.
We take a closer look at these semantically close set of words, and confirm by connecting back to the global context of the embeddings through the \emph{neighborhood distance view} and the \emph{density view} that those are clusters that are particularly close within both embeddings.


Also in the list of stable words are kinship terms, which also form a tight cluster in the both embeddings.
We select them in the selection list table and view their positions in the \emph{scatterplot view} with t-SNE dimensionality reductions, expecting them to cluster together.
In the view of the Wikipedia embedding, all points are close together except for one, which hovering reveals as ``parent''.
Focusing on ``parent'', the \emph{neighbor list view} shows that the neighbors in the Wikipedia embedding reflect its use in the sense of ``parent company'', including words such as \emph{subsidiary} and \emph{acquisition}. In contrast, parent's neighbors in the EBBO embedding are family terms such as sister and brother.

% This is a good example, but it doesn't add much
% We then focus on the split cluster in the eebo embedding.
% By viewing the nearest neighbors, we notice that while the terms in the one cluster only have other kinship terms close to them, terms in the second cluster, including \emph{uncle}, \emph{nephew}, and \emph{grandfather} also have hearest neighbors that seem to be related to the order of succession for nobility titles.
% Example include \emph{predecessor} and \emph{successor}.
% We can thus conclude that some of the kinship terms appear more often in the context of succession of nobility titles within eebo, resulting in those two clusters.

Selecting objects with low overlap (zero overlaps in the 50-neighborhood) leads to another selection of words which we would expect to have changed meanings.
On this list, we were surprised to find \emph{cup}, whose common meaning should be stable.
However, in investigating the word in \emph{neighbor list view}, we see that while in EEBO its neighbors reflect its common meaning as a drinking vessel, the neighbors in Wikipedia reflect its alternate modern usage as a trophy.

After the initial sessions, we had additional meetings with the experts.
They were very interested in comparing more historic and contemporary corpora, including subsets of EEBO and embeddings built from the Google ngrams corpus.
During those comparisons, they were able to uncover a range of additional insights about change in the English language over time.

